Deciphering the Factors Influencing the Efficacy of Chain-of-Thought: Probability, Memorization, and Noisy Reasoning

Chain-of-Thought (CoT) prompting has been shown to enhance the multi-step reasoning capabilities of Large Language Models (LLMs). However, debates persist about whether LLMs exhibit abstract generalization or rely on shallow heuristics when given CoT prompts. To understand the factors influencing CoT reasoning we provide a detailed case study of the symbolic reasoning task of decoding shift ciphers, where letters are shifted forward some number of steps in the alphabet. We analyze the pattern of results produced by three LLMs -- GPT-4, Claude 3, and Llama 3.1 -- performing this task using CoT prompting. By focusing on a single relatively simple task, we are able to identify three factors that systematically affect CoT performance: the probability of the task's expected output (probability), what the model has implicitly learned during pre-training (memorization), and the number of intermediate operations involved in reasoning (noisy reasoning). We show that these factors can drastically influence task accuracy across all three LLMs; e.g., when tested with GPT-4, varying the output's probability of occurrence shifts accuracy from 26% to 70%. Overall, we conclude that CoT prompting performance reflects both memorization and a probabilistic version of genuine reasoning. Code and data at this https://github.com/aksh555/deciphering_cot

==> section/checklist.tex <==
\section*{NeurIPS Paper Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and precede the (optional) supplemental material.  The checklist does NOT count towards the page
limit. 

Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
\begin{itemize}
    \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
    \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
    \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
   % \item {\bf The papers not including the checklist will be desk rejected.}
\end{itemize}

{\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

IMPORTANT, please:
\begin{itemize}
    \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS paper checklist"},
    \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
    \item {\bf Do not modify the questions and only use the provided macros for your answers}.
\end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Claims made in the abstract and introduction are based on the results we obtain and have been justified.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: See \autoref{sec:conclusion} Limitations and future directions. 
    \item[] Guidelines: 
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We do not have any theoretical proofs.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: See \autoref{sec:exp_details}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: See \autoref{sec:exp_details} and \autoref{ss:word_dataset}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: See \autoref{ss:word_dataset}. We manually checked the words in the dataset and filtered them to ensure there were no inappropriate words used.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We do not crowdsource or research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We do not crowdsource or research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}


==> section/old_experiment.tex <==
\section{Experiments}
\label{sec:experiment}

\begin{figure}
\centering
        \includegraphics[width=\textwidth]{figures/overall_vs_step_acc_text_cot.pdf}
        \caption{\small \textbf{Actual} \textcolor{blue}{overall decoding accuracy} vs. \textcolor{orange}{step accuracy} across shift levels showing the hallmarks of \textit{noisy reasoning}, \textit{memorization}, and \textit{probabilistic reasoning}. The probabilistic effect is exhibited by a drop in accuracy from \textcolor{orange}{step outputs curves} to the \textcolor{blue}{overall answer curves}. The effect is amplified for low probability outputs as seen in the large spread in overall accuracies between \textcolor{blue}{\texttt{bin 1} (high prob)} and \textcolor{blue}{\texttt{bin 5} (low prob)} lines.}
\label{fig:overall_vs_step_acc_text_cot}
\end{figure}

\begin{figure}
\centering
        \includegraphics[width=\textwidth]{figures/overall_vs_concat_steps_vs_step.pdf}
        \caption{\small \todo{fix this}}
\label{fig:fix}
\end{figure}

\subsection{Disentangling the factors involved in decoding shift ciphers}
\label{ss:cot_factors}
GPT-4's shift cipher performance displays hallmarks of several different types of reasoning
(\autoref{fig:overall_vs_step_acc_text_cot}).
First, accuracy generally decreases as the shift level increases, a hallmark of noisy reasoning. Note that GPT-4's performance is, in particular, indicative of a two-way version of noisy reasoning in which it can decode a message by shifting letters forward or backward (e.g., a shift level of 1 can be decoded by shifting back 1 letter, while a shift of 25 can be decoded by shifting forward 1 step, as doing so requires fewer steps than shifting backward 25 steps); this two-way nature shows up in the way that accuracy increases as the shift level changes from 20 to 25.

Second, evidence of probabilistic reasoning can be seen in the fact that accuracy is substantially higher for \texttt{bin 1} (the highest-probability bin) than \texttt{bin 5} (the lowest-probability bin).
%highlights how the noisy two-way reasoning, memorization, and probabilistic reasoning types detailed in \autoref{ss:reasoning_formulation} and shown in \autoref{fig:reasoning}, culminate in the observed overall decoding accuracy curve in blue.
Finally, although a shift level of 13 requires the most reasoning steps of any shift level (under the assumption that decoding can be done in a forward or backward direction), there is a major spike in accuracy at a shift level of 13. As discussed above, this spike is a hallmark of memorization since 13 is the most common shift level in natural corpora.
%and being the most noisy, the memorization effect notably enhances the model's performance. While probabilistic effects may not be conspicuous at the step-level due to the output being a single letter (as seen , their impact becomes evident at the overall level, as evidenced by the substantial variance between \texttt{bin 1} and \texttt{bin 5}.
%This illustrates the hallmarks of noisy reasoning, memorization, and probabilistic reasoning. 

\textbf{A simple probabilistic approach to modeling the reasoning process. }
\label{sec:method_lr_model}
To make these intuitively-stated observations more rigorous, we perform a logistic regression to determine the statistical significance of several factors on performance. 
The outcome variable is a binary variable indicating whether GPT-4 got the correct answer on each example. We include the following predictor variables: 
\begin{itemize}[nosep]
    \item $input\_logprob$ - the log probability of the encoded input text as measured by GPT-2 \cite{radford2019language}. The inputs tend to have a very low probability because they are enciphered.  
    % (Figure~\ref{fig:encoded_stimuli_logprob}).
    \item $output\_logprob$ - the log probability of the expected ground-truth output text as measured by GPT-2. 
    \item $shift\_freq$ - we used the frequency of occurrence of all shift levels that \cite{mccoy2023embers} provided; that paper derived these frequencies through manual analysis of the C4 corpus \cite{raffel2020exploring}. The assumption is that the distribution of shifts in C4 is similar to the distribution of shifts in the training data for GPT-4.
    \item $\min (shift\_level,26-shift\_level)$ - this value is the minimum number of steps that must be performed to decode each letter, under the assumption that decoding can be done by moving $shift\_level$ steps backward or $(26 - shift\_level)$ steps backward; as discussed above, GPT-4 indeed shows evidence of using both of these decoding directions.
    \item $output\_num\_chars$ - number of characters in the output word. By construction this is 7.
    \item $output\_num\_tokens$ - number of tokens in the output word. By construction this is 2.
\end{itemize}

\todo{keep/cut? Decoding shift ciphers with CoT involves:
\begin{enumerate}[nosep]
\item copying the input letters from the encoded input in corresponding reasoning steps,
\item given the input letter for a reasoning step, producing the output letter for that step,
\item generating the final answer by concatenating outputs from all the reasoning steps.
\end{enumerate}
Step 1 is done accurately by advanced models like GPT-4. The accuracy of steps 2 and 3 are influenced by 
\begin{itemize}[nosep]
\item the probability of occurrence of the expected output  (\autoref{ss:prior_effects}),
\item its ease to decode smaller shift levels and attempts to adopt shorter alternate reasoning paths making the reasoning noisy (\autoref{ss:noise_effects}), 
\item what shift levels the model has encountered more during its pre-training (\autoref{ss:memorization_effects}),
\item and whether the model explicitly generates helpful step outputs (\autoref{ss:hidden_reasoning}).
\end{itemize}}

Several of these variables correspond to the critical properties that are indicative of the reasoning processes that we have hypothesized: $output\_logprob$ should have a significant effect if probabilistic reasoning is used, $shift\_freq$ should have a significant effect if memorization is used, and $\min (shift\_level,26-shift\_level)$ should have a significant effect if noisy reasoning is used. The remaining factors are included as potential confounds to control for.
The overall logistic regression that we ran thus took the following form:
\begin{equation}
\label{eq:logistic_reg}
\begin{aligned}
& correct   \sim   \min (shift\_level,26-shift\_level) \\ & \qquad\qquad + input\_logprob + output\_logprob  + shift\_freq
\end{aligned}
\end{equation}
The intuition for using $\min (shift\_level,26-shift\_level)$ arises from the observation that LMs try to adopt shorter reasoning paths (see Figures~\ref{fig:overall_vs_step_acc_text_cot}, \ref{fig:text_math_plot2_20-23}).

\textbf{Logistic regression results}
Under our logistic regression, the following features had a statistically significant effect on model performance: $output\_logprob$, $shift\_frequency$, and $\min (shift\_level,26-shift\_level)$.
These results therefore quantitatively support the conclusion that GPT-4 incorporates processes based on probability, memorization, and noisy reasoning.
%We associate $output\_logprob$ to model the probabilistic effect, $shift\_frequency$  to model memorization, and $shift\_level$ to model the noise. 
\autoref{fig:lr_plot} shows the predictions of the logistic regression compared to GPT-4's actual performance. 
The logistic regression correctly predicts the main trends in GPT-4's behavior (as expected, it does not match the curve exactly due to the simplicity of the logistic regression model). 

In the next several subsections, we conduct some additional experiments that investigate each hypothesized reasoning process in more detail.
%Given the limited training set we collect and the simplistic nature of the model, it is able to roughly capture the trend.
% Additional auxiliary plots are shown in Appendix \S~\ref{appx:experiments:lr} Figure~\ref{fig:lr_plots}.

\begin{figure}
    \centering
\includegraphics[width=0.7\textwidth]{figures/text_cot_lr.pdf}
    \caption{\small Logistic Regression to model GPT-4's performance on the shift cipher task across all probability bins. The \textcolor{green!50!black}{logistic regression curve} captures the overall trend exhibited by \textcolor{blue}{GPT-4}. The other curves are ablations of using logistic regressions with only one feature among $output\_logprob$, $shift\_freq$, $shift\_level$  to show individual effects.}
    \label{fig:lr_plot}
\end{figure}

\subsection{Analyzing the effect of probability}
\label{ss:prior_effects}
% We understand the prior effect by choosing sentences from different bins of likelihood of occurrence as the expected decoded outputs. Encoding in general produces words that are of low probability as seen in \S~\ref{appx:experiments:math_only_prompt} Figure~\ref{fig:encoded_stimuli_logprob}. 

In this section, we collect more evidence of the probabilistic effect. If probability does play a role, we can expect to observe unfaithfulness of a particular sort -- helpful unfaithfulness when the correct answer is high probability and unhelpful unfaithfulness when the correct answer is low probability. So, let's check this. In our new figure, we indeed see these trends!

As noted above, 
%Although the algorithm for decoding could in principle be the same for any input, we note from 
\autoref{fig:overall_vs_step_acc_text_cot} shows that the overall decoding accuracy is much lower for output texts having a low probability of occurrence (the gap between \texttt{bin 5} vs. \texttt{bin 1} lines in blue). 
In addition, there is another result shown in this plot that may also relate to probability, namely unfaithfulness. Unfaithfulness occurs when an LLM produces a chain of thought followed by a final answer that does not match the chain of thought. 
Mathematically, this plot shows the difference between $P(correct\_step\_output \mid shift\_level)$ and $P(correct\_final\_output \mid shift\_level)$.
The consequent \textit{unfaithfulness} aspect is also captured by an average 72\% relative drop in accuracy compared to producing the step-level outputs accurately and concatenating them to form the final answer when averaged across all shift levels and probability bins.
\autoref{tab:unfaithfulness} more concretely analyzes the unfaithfulness in CoT due to the flip effects of the output's probability. On average, incorrect intermediate chains yield correct answers 44\% times in high probability but just 10\% times in low probability. On the other hand, correct intermediate chains result in incorrect answers 4\% times in high probability outputs but 12\% times in low probability outputs.
\input{tables/unfaithfulness}
\textit{This establishes that models over-rely on their prior knowledge \cite{jang2023can}  thereby introducing biases in their outputs. If the answer has a high probability of occurrence, the model's priors favor generating it even if its intermediate reasoning steps suggest an alternative output. Conversely, if the answer is of lower likelihood, then even if the chain of reasoning is correct, the priors exert a detrimental influence causing wrong answer generations.}

% \todo{Noise is lower in situations with high priors? how to show this?}


\subsection{Analyzing the noise effect}
\label{ss:noise_effects}
The statistically significant impact of $shift\_level$ can be viewed as evidence that GPT-4's CoT behavior is in part a noisy version of symbolic reasoning. 
%Smaller shifts are done easily, due to fewer backward shift operations required in every reasoning step, as seen in 
%the falling accuracy values from \texttt{rot-1} to \texttt{rot-12} and it is two-way as higher shift levels recover in \autoref{tab:text_vs_math_cot}.
Accuracy falls as the shift level increases from 1 to 12 and then recovers at higher shift levels \autoref{tab:text_vs_math_cot}, consistent with a noisy reasoning process in which deciphering a shift level of $n$ involves $\min (n,26-n)$ steps, with noise that gives each step some probability of being performed incorrectly.

\begin{wrapfigure}[16]{r}{0.5\textwidth}
\vspace{-.5cm}
\includegraphics[width=0.5\textwidth]{figures/text_math_plot2_20-23.pdf}
\caption{\small Normalized frequency distribution vs. predicted $shift\_level$ of step answers for \texttt{rot-20} to \texttt{rot-23}. The appearance of peaks at $26 - shift\_level$ in \textcolor{pink}{Math-CoT} and \textcolor{green!50!black}{Text-CoT} prompts showing the model's noisy attempt in taking the shorter reasoning path i.e. $26-x$ shifts forward instead of $x$ backward.}\label{fig:text_math_plot2_20-23}
\end{wrapfigure}

% \begin{figure}
%     \centering
% \includegraphics[width=0.7\textwidth]{figures/text_math_plot2_20-23.pdf}
%     \caption{Normalized frequency distribution vs. predicted $shift\_level$ of step answers for \texttt{rot-20} to \texttt{rot-23}. The appearance of peaks at $26 - shift\_level$ in \textcolor{pink}{Math-CoT} and \textcolor{green!50!black}{Text-CoT} prompts showcasing the model's noisy attempt in taking the shorter reasoning path i.e. moving $26-x$ shifts forward instead of $x$ backward.}
%     \label{fig:text_math_plot2_20-23}
% \end{figure}

\textbf{Tendency to adopt shorter reasoning paths. } 
We have argued that the relation between accuracy and shift level is evidence for a two-way strategy being used by GPT-4. That is, accuracy is high for small shifts such as 1 but also for large shifts such as 25, which could plausibly be explained by GPT-4 decoding by implicitly selecting whichever direction will minimize the number of steps it needs to compute---shifting letters backward for small shift levels or forward for large shift levels.
This two-way strategy is effective in that it supports strong performance on large shift levels such as 25. 
However, we also observe evidence that it contributes to the noise that causes accuracy to decline as the shift level increases.
\autoref{fig:text_math_plot2_20-23} shows the actual shift level that GPT-4 produces for each letter in its chain of thought, for each of the four intended shift levels. Across all four of these cases, GPT-4 shows peaks at both $shift\_level$ and $26 - shift\_level$.
Thus, while some of the noise affecting the reasoning process may be random, it appears that at least some of the noise can be attributed to confusion between possible shift levels. Decoding a shift level of $n$ can be done by shifting backward $n$ steps or forward $26-n$ steps, but it appears that GPT-4 sometimes mixes up these two strategies by shifting forward $n$ steps (or, equivalently, shifting backward $26-n$ steps), contributing to the overall noise.
%There is an interesting emerging phenomenon as seen in \autoref{fig:text_math_plot2_20-23}; for large $shift\_level$, the emergence of additional peaks at $26 - shift\_level$ in both text and math cases. 
%It looks like the model has understood the equivalence between $x$ shifts backward and $26 - x$ shifts forward; but in the attempt to take a shorter reasoning path, it is still affected by the demonstration showing backward shifting, possibly giving rise to these peaks. This noise is very prevalent until \texttt{rot-23} after which the model performs similarly to \texttt{rot-1} and \texttt{rot-2}. 
% Plots across all shift levels can be found in Appendix \S~\ref{appx:experiments:plot2}.

\todo{AP - keep this? \paragraph{Discretization property.}
In standard prompting, the LM produces the output in one go based on simple next-token prediction. For both low and high temperature settings, CoT does better than standard prompting probably because it produces the intermediate answers in the form of steps in the chain independently; rather than in standard prompting where every step answer is implicitly conditioned on the generation thus far. 
The prevalence of this property only for CoT is not clear. If we have arroy / arrow examples and show that CoT predicts arroy while standard predicts arrow then it is more convincing. But these could be hampered by prior effects as in low prob cases? maybe we can show something like in standard its even more harder to predict a low prob word than CoT because of the auto-regressive nature of predicting in one go rather than CoT where step answer are correct and only prior effect of combining could happen
This makes us believe that CoT does well as it discretizes the internal probability distribution of the model. But CoT is not pure reasoning; increasing temperature introduces more noise similar to standard prompting.}


\subsection{Analyzing the memorization effect}
\label{ss:memorization_effects}
A shift level of 13 is by far the most frequently occurring shift level in the corpora analyzed by \cite{mccoy2023embers}, and we observe in \autoref{tab:text_vs_math_cot} that GPT-4 shows a spike in accuracy at this shift level in both text-based and math-based CoT. Even with just standard prompting, GPT-3.5 and GPT-4 have been found to perform significantly better for such shifts \cite{mccoy2023embers} and they attribute it to task probability. The aforementioned property of \textit{unfaithfulness} also partly demonstrates this effect. A comparison between \autoref{tab:rot13-unfaithfulness} and \autoref{tab:rot4-unfaithfulness} shows how in the more frequently encountered \texttt{rot-13}, despite incorrect chain step outputs, the final answer is accurate on average \textbf{twice} as often for \texttt{rot-13} compared to \texttt{rot-4}.

It is more likely that the model has seen the alphabet in the forward direction due to which it finds it harder to go backward in the alphabet and circle backward from a to z. Using our two prompting styles helps us verify this as when we remove the model's dependence on its memory of the alphabet in the Math-CoT case by providing a definite formula, the model consistently does better across most shift levels (see \autoref{tab:text_vs_math_cot}).
\input{tables/text_vs_math_cot}


\subsection{Producing explicit reasoning steps and impact of their validity \footnote{Prompts used are shown in \S~\ref{appx:experiments:hidden_prompt} Figure~\ref{fig:hidden_prompts} and \S~\ref{appx:experiments:desc_demo} Figure~\ref{fig:desc_demo_prompt}}}
\label{ss:hidden_reasoning}

\todo{motivation}Prior works 

\textbf{Strong reliance on the surface strings produced in reasoning steps. }

\textbf{1. Using hidden chain. } In this case, we use the Text-CoT prompt but instruct the model to \textit{not reveal step answers and instead output a *}. The step answers in the demonstration are also replaced by `*' - thus we leave the format of reasoning intact but the expected generation token has changed. When tested, the performance is similar to that of standard prompting.

\textbf{2. Using partially hidden chain. }
Next, we ask the model to explicitly \textit{think about the correct letter that should go in the place of the star but just not write it down}. In the demonstration, we first provide an example with all step answers and then replace with * to guide the model. But even this does not rescue the model.

\textit{This supports the view that CoT is more about “self-conditioning” - it needs to explicitly produce these relevant step outputs, that later predictions can be conditioned on to generate the final answer. Merely instructing a model to \q{think} silently is not helping, proving that the reasoning is not an intrinsic process.}

\textbf{Unnaturalness phenomenon: Description vs. demonstration. }
% All prompts variants are displayed in \S~\ref{appx:experiments:desc_demo}
% Figure~\ref{fig:desc_demo_prompt}.

\textbf{1. Random corruptions.}
Here the step answers in the demonstration are replaced by a random letter -- both format and expected generation token (a letter) are left unchanged.

\textbf{2. Systematic mismatches.}
The description for \texttt{rot-13} is provided while the demonstration is that of \texttt{rot-14}. This can be viewed as a systematic \q{helpful} corruption as it still retains the overall format and expected generation token (a letter) for every step in the chain. 

% We experiment with both text-based and math-based CoT prompts. There is a subtle difference - the math-based CoT even though shows a demonstration of a different $shift\_level$ than the description, explicitly mentions it in the reasoning step.

In none of these cases (i.e. random or systematic corruption) is the model severely distracted from the description, the converse was observed with GPT-3 \cite{rong2021extrapolating,jang2023can}. This reinforces the fact that there is no strong correlation between the validity of the reasoning shown in the demonstration and the model performance \cite{wang-etal-2023-towards, madaan2022text, ye-etal-2023-complementary}. The demonstration seems to merely guide the model to solve the task by providing a format to generate accurate reasoning steps \cite{wang2024chainofthought}. 
\textit{As long as the model can produce relevant step outputs to self-condition on, and is provided with a relevant demonstration \cite{wang-etal-2023-towards} that could be invalid as well, it improves over standard prompting, biased by the prior, memorization and noise effects previously described.}

% When the pattern of the corruption is explicitly present in the demonstration/description as in the case with the math-based CoT prompt (where the $shift\_level$ being followed is mentioned in both) or when the pattern is not explicit as in the case with the text-based CoT prompt, (where the $shift\_level$ being followed is not mentioned in the demonstration directly or in the case of random corruption when the pattern is non-deterministic) the model always tries to follow the description. , the corruption  but still does not break down the format, so the model falls back to relying on the description, without much loss in performance.

==> section/old_experiment_details.tex <==
\section{Experimental details}
\label{sec:exp_details}
\subsection{Data}
\label{ss:word_dataset}
% \label{ss:data}
% The dataset for decoding shift ciphers has data categorized into \texttt{high, medium, low} probability bins each containing 100 sentences. The high probability sentences are drawn from GlobalVoices \footnote{\url{https://globalvoices.org/}} news articles (dated between June 2, 2023 to June 16, 2023), and select the first 100 sentences ranked in increasing order of maximum perplexity of any token in that sentence. The medium-probability set was created by taking the high-probability sentences and using RoBERTa \cite{liu2019roberta} to substitute some words with other alternates that had a low probability of occurrence in that context (but were still grammatical). Each replacement word was required to be the same length as the word it was replacing, in terms of both the number of letters or sub-word tokens. The low-probability set was created by randomly shuffling the words of the medium-probability examples, except retaining the first and last words in their positions.

We construct a dataset comprising 7-letter words having exactly 2 tokens (measured using the tokenizer used by GPT-4) to control for confounding factors relating to tokenization. Specifically, we find all 3-letter and 4-letter tokens from the lowercase English alphabet and form words by considering all possible combinations of a 3-letter and 4-letter token.
The words are scored by their log probability and arranged in descending order. Subsequently, five bins are formed by selecting equidistant log probability values as centers. Following this, 150 words (100 used to train, 50 to test) with log probability values nearest to each respective center are allocated into 5 distinct bins \texttt{\{bin1, bin2, bin3, bin4, bin5\}}, i.e. \texttt{bin1} meant high probability and \texttt{bin5} meant low probability. 
Following \cite{mccoy2023embers}, we compute the log probability as the log probability that GPT-2 \cite{radford2019language} assigns to the sentence `\texttt{The word is "WORD"}', minus the log probability that it assigns to `\texttt{The word is "}'; thus, this yields the log probability assigned to just the word and the following quotation mark in the context of `\texttt{The word is "}'. The closing quotation mark is included because it indicates the end of the word. We manually checked the words in the dataset and filtered them to ensure there were no inappropriate words used.


\subsection{Prompting styles}
Refer \autoref{fig:text_math_cot_prompts} for prompts used. The description of the task at hand is common across all styles. \\
\textbf{Text-based chain of thought.}
We adopted this version of the prompt involving text, guided by insights from \cite{mccoy2023embers}, which tried several variants and found this to be the best. To get a reasoning step correct, the model must have learned the alphabet during pre-training.
\\
\textbf{Math-based chain of thought.}
% \input{tables/math_cot_prompt}
The prompt utilizes arithmetic skills in the reasoning steps eliminating the need for the model to know the alphabet ordering as the letter-position mapping is specified. 
\\
\textbf{Standard.} This is a prompt with just the description provided and no demonstration.
\input{tables/text_math_cot_prompt} 
Except where otherwise stated, the prompt style we use throughout is text-based CoT as it effectively helps us observe and analyze all the factors involved in the reasoning factors. 

\subsection{Model}
We run experiments using OpenAI's GPT-4 (\texttt{gpt-4-0613} version) that is state-of-the-art in many areas, setting \texttt{temperature} to $0$ and \texttt{max\_new\_tokens} to $200$. Using GPT-4 helps us to control several sources of noise making it easier to focus on the task itself and isolate the factors affecting CoT. It ensures that the format of the demonstration is closely followed, and copy errors are avoided/minimal (correctly copying the letter from encoded text input in the reasoning steps and the prompt metadata such as the letter-position mapping).

==> section/old_methods.tex <==
\section{Formulation}
\label{sec:methods}

\subsection{The puzzling status of CoT reasoning}
\label{ss:background}
Our experiments are based on shift ciphers -- a type of simple strategy for encoding text. Encoding a message with a shift cipher involves replacing every letter with another letter that is some fixed number of positions (called $shift\_level$) forward in the alphabet; decoding is the reverse (shifting backward) as shown in \autoref{fig:preview}. For example, given the test word \q{FDW} and that  \texttt{rot-3} encryption has been used ($shift\_level = 3$), decoding involves shifting every letter $3$ steps backward, i.e. \textit{F $\rightarrow$ C}, \textit{D $\rightarrow$ A}, and \textit{W $\rightarrow$ T} to obtain \q{CAT} as the output.
%It falls under the category of symbolic reasoning as it involves the manipulation of abstract symbols according to a formal rule. 
In our experiments, we give an LLM a single word that has been encoded with a shift cipher and ask it to decode this text to recover the original word.

\autoref{fig:preview} provides some basic initial results that will help us motivate why we chose this family of tasks.
GPT-4 \cite{openai2024gpt4} out of the box gets zero accuracy across most shift levels, but it improves substantially (to an average accuracy of 32\%) when CoT prompting is used; this result replicates the finding in \cite{mccoy2023embers} that CoT is helpful for shift ciphers.
However, the performance with CoT remains far from perfect. When we use an alternative task that is isomorphic to shift ciphers but based on number sequences instead of letter sequences, GPT-4's performance becomes nearly perfect (more details are in \autoref{appx:experiments:math_only_prompt}).

These results paint CoT prompting in a puzzling light. The isomorphic number-based task shows that GPT-4 has the core reasoning abilities that would be needed to decode shift ciphers perfectly. Thus, if CoT prompting led to symbolic reasoning, GPT-4 would score perfectly. The fact that it does not, shows that CoT reasoning is not pure symbolic reasoning. Nonetheless, it is also clear that CoT does substantially improve over standard prompting, so it is unlikely that CoT reasoning can be explained away as simple memorization.


%\textbf{Isolating the reasoning process. }
%To assess the model's performance on only the decoding task without being influenced by any effects, we create a version of the problem by abstracting out the alphabet where input and output are now number sequences where the elements are the positions of the corresponding letters of the input and output messages respectively in the alphabet. The full prompt, and related error analysis are shown in \autoref{appx:experiments:math_only_prompt}
% Figure~\ref{fig:math_only_acc} 
%The model's near-perfect accuracy across shift levels implies that the model is in fact very strong in the core reasoning needed for decoding shift ciphers. However, when the same task is shifted to the alphabet domain, it is impacted by several effects discussed in \autoref{ss:cot_factors}. 

%\textbf{Motivation. } 
%From \autoref{fig:preview}, it is clear that CoT is doing something helpful for some shift levels, but that it’s still not getting the model to the level that it should be able to perform (close to the number sequence case). 
\textit{\q{If an LLM's CoT behavior is neither simple memorization nor pure reasoning, what is it?}} 
This question is the focus of our paper. In the rest of this section, we introduce several types of reasoning that CoT could involve and describe why shift ciphers are a useful testbed for disentangling these types of reasoning. The following sections then describe our experimental setup, including the setup for the initial results described above (\autoref{sec:exp_details}), followed by our detailed results (\autoref{sec:experiment}).
%(2) why does it help and why does it sometimes still fail? (3) what are the important aspects aiding it?

\subsection{Probabilistic memorization influenced noisy reasoning}
\label{ss:reasoning_formulation}
We consider four types of reasoning processes.

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/hypo_reasoning.pdf}
        \caption{\small \textbf{Hypothetical} accuracy vs. shift-level for various types of reasoning. \textcolor{lightorange}{Noisy one-way} considers the model knows only going forward a-z; \textcolor{orange}{noisy two-way} considers the model adopts the shorter path between going forward and backward. \textcolor{darkgreen}{Memorization} is based on shift levels observed in internet corpora. \textcolor{blue}{Probabilistic} would imply high probability (\textcolor{blue}{\texttt{bin 1}}) is much better than low probability (\textcolor{blue}{\texttt{bin 5}}).}
        \label{fig:reasoning}
\end{figure}

% \begin{figure*}[htbp]
%     \centering
%     \begin{minipage}[b]{0.48\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/hypo_reasoning.pdf}
%         \caption{\textbf{Hypothetical} accuracy vs. shift-level for various types of reasoning. \textcolor{lightorange}{Noisy one-way} considers the model knows only going forward a-z; \textcolor{orange}{noisy two-way} considers the model adopts the shorter path between going forward and backward. \textcolor{darkgreen}{Memorization} is based on shift levels observed in internet corpora. \textcolor{blue}{Probabilistic} would imply high probability (\textcolor{blue}{\texttt{bin 1}}) is much better than low probability (\textcolor{blue}{\texttt{bin 5}}).}
%         \label{fig:reasoning}
%     \end{minipage}
%     \hfill
%     \begin{minipage}[b]{0.48\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/overall_vs_step_acc_text_cot.pdf}
%         \caption{\textbf{Actual} \textcolor{blue}{overall decoding accuracy} vs. \textcolor{orange}{step accuracy} across shift levels showing the hallmarks of "noisy reasoning", "memorization", and "probabilistic reasoning". The probabilistic effect is exhibited by a drop in accuracy from \textcolor{orange}{step outputs curves} to the \textcolor{blue}{overall answer curves}. The effect is amplified for low probability outputs as seen in the large spread in overall accuracies between \textcolor{blue}{\texttt{bin 1}} and \textcolor{blue}{\texttt{bin 5} lines}.}
%         \label{fig:overall_vs_step_acc_text_cot}
%     \end{minipage}
% \end{figure*}


\begin{enumerate}[label=(\alph*),noitemsep,topsep=0pt]
\item \textbf{Symbolic reasoning} is the use of discrete, deterministic inference rules. Shift ciphers can be perfectly decoded with a simple symbolic algorithm, so a system using fully systematic reasoning, should attain 100\% accuracy on all shift cipher examples.
\item \textbf{Noisy reasoning} is like symbolic reasoning but with the addition of noise that introduces some possibility of each intermediate operation in a reasoning step being wrong. Thus, if the system uses noisy reasoning, we should see accuracy decrease as we increase the number of operations that need to be performed. Shift ciphers let us test this possibility: by varying $shift\_level$, we can modulate the number of operations that need to be performed in every reasoning step, and observe if accuracy decreases as the number of operations increases.
\item \textbf{Memorization} is a strategy in which a system memorizes the tasks it has encountered in pretraining but does not generalize to new tasks. If memorization is all that's happening, we should see higher performance in the cases that are frequently encountered during pre-training than the ones that are not. Prior work \cite{mccoy2023embers} has shown that $13$ is by far the most common shift level in natural corpora because this shift level (sometimes called \texttt{rot-13}) is popular in some online communities. Thus, a hallmark of memorization would be much higher accuracy at $13$ than other shift levels.
%This is one of the strongest reasons for using shift ciphers because they allow us to disentangle \q{difficulty} from \q{frequency in pre-training}.
\item \textbf{Probabilistic reasoning} frames a task as choosing the output that is most probable given the input. Such reasoning would be influenced by the prior probability of the output: a probabilistic reasoner should show accuracy that increases as the prior probability of the correct answer increases.
%: As the probability of the correct output decreases, accuracy should also decrease. Shift ciphers are also ideal for testing this because the output can be any string we want -- allowing us to modulate the probability easily.
\end{enumerate}

\autoref{fig:reasoning} spotlights the hypothetical performance trends that would be observed in a system adopting each of these reasoning approaches. These processes are not mutually exclusive. For instance, a reasoner could be influenced by both probability and memorization. Indeed, to preview our results, we will be arguing that GPT-4's CoT performance involves noisy reasoning, memorization, and probabilistic reasoning because its performance in \autoref{fig:preview} displays the hallmarks of all three strategies.




==> tables/text_vs_math_cot.tex <==
\begin{table*}
  \centering
  \resizebox{\textwidth}{!}{%
  \begin{tabular}{*{26}{l}}
    \toprule
    Style / Shift Level & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 & 16 & 17 & 18 & 19 & 20 & 21 & 22 & 23 & 24 & 25 \\
    \midrule
    Text CoT & \textcolor{blue}{49.2} & \textcolor{blue}{52.4} & \textcolor{blue}{50.8} & 51.6 & 42.8 & 47.0 & 32.6 & 44.0 & 30.2 & 9.6 & 0.2 & 0.0 & \textcolor{blue}{60.0} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & \textbf{16.6} & \textbf{17.0} & \textbf{47.0} & 45.4 & 50.4
 \\
    Math CoT & \textcolor{blue}{\textbf{70.2}} & \textcolor{blue}{\textbf{68.0}} & \textcolor{blue}{\textbf{68.6}} & \textbf{66.2} & \textbf{58.8} & \textbf{60.4} & \textbf{57.4} & \textbf{63.2} & \textbf{45.4} & \textbf{41.6} & \textbf{40.2} & \textbf{33.8} & \textcolor{blue}{\textbf{71.0}} & \textbf{16.2} & \textbf{19.2} & \textbf{17.8} & \textbf{11.4} & \textbf{8.8} & \textbf{4.8} & \textbf{1.6} & 0.8 & 0.6 & 0.0 & \textbf{50.0} & \textbf{61.6}
\\
    \bottomrule
  \end{tabular}}
  \caption{Accuracy for Text- and Math- CoT prompt styles with GPT-4. Math-CoT performs better than Text-CoT, but both display evidence of memorization as accuracy is highest for \textcolor{blue}{shift level 13} ---the most frequent shift in real-world corpora.
  %Implicit need for memorization in Text-CoT causes an overall reduced performance. Model performs best at \textcolor{blue}{shift levels 13, 1, 3, and 2} which are the most frequent shifts in real-world corpora highlighting memorization.
  }
  \label{tab:text_vs_math_cot}
\end{table*}
